E2ED^2:Direct Mapping from Noise to Data for Enhanced Diffusion Models

Diffusion models have established themselves as the de facto primary paradigm in visual generative modeling, revolutionizing the field through remarkable success across various diverse applications ranging from high-quality image synthesis to temporal aware video generation. Despite these advancements, three fundamental limitations persist, including 1) discrepancy between training and inference processes, 2) progressive information leakage throughout the noise corruption procedures, and 3) inherent constraints preventing effective integration of modern optimization criteria like perceptual and adversarial loss. To mitigate these critical challenges, we in this paper present a novel end-to-end learning paradigm that establishes direct optimization from the final generated samples to initial noises. Our proposed End-to-End Differentiable Diffusion, dubbed E2ED^2, introduces several key improvements: it eliminates the sequential training-sampling mismatch and intermediate information leakage via conceptualizing training as a direct transformation from isotropic Gaussian noise to the target data distribution. Additionally, such training framework enables seamless incorporation of adversarial and perceptual losses into the core optimization objective. Comprehensive evaluation across standard benchmarks including COCO30K and HW30K reveals that our method achieves substantial performance gains in terms of Fr\'echet Inception Distance (FID) and CLIP score, even with fewer sampling steps (less than 4). Our findings highlight that the end-to-end mechanism might pave the way for more robust and efficient solutions, \emph{i.e.,} combining diffusion stability with GAN-like discriminative optimization in an end-to-end manner.

==> sec/2_related_work_bk.tex <==
\section{Related Work}

% \noindent \textbf{Denoising Diffusion Probabilistic models.} Denoising Diffusion Probabilistic Models (DDPMs), introduced by Ho et al.\cite{ho2020denoising}, have significantly transformed the landscape of generative modeling by enabling high-quality image generation through an iterative refinement process. The core mechanism of DDPMs involves gradually denoising an image, which effectively maintains high image quality across various datasets, including ImageNet (Deng et al., 2009). This ability to preserve image quality while enhancing sampling efficiency has established a new benchmark in the field.

% \noindent \textbf{Flow.} Building on the capabilities of DDPMs, Normalizing Flows, introduced by Rezende and Mohamed (2015), have advanced the field by enabling the modeling of complex distributions with simpler, invertible transformations. These transformations facilitate precise likelihood calculations and more efficient sampling, thereby accelerating the training process and supporting more dynamic generative applications. The integration of Normalizing Flows with DDPMs has not only improved model flexibility but also expedited adaptation to diverse data modalities.

% \noindent \textbf{Diffusion Transformer.} The Transformer architecture, introduced in 2017, has significantly advanced language processing and expanded its utility to a broad spectrum of computer vision tasks, such as image classification, object detection, and semantic segmentation. Building on these successes, the Diffusion Transformer (DiT) model employs transformer technology to supplant the conventional convolutional U-Net backbone. This adaptation not only enhances the model's scalability but also boosts its parameter efficiency, positioning it as a potent solution for complex generative tasks. Notably, the DiT has excelled in converting text to high-quality images, underscoring its capability as a pivotal model for the development of real-time generative applications.


\subsection{Diffusion Models} % DDPM, SMLD, flow , DiT....
Denoising Diffusion Probabilistic Models (DDPMs) introduced by Ho et al. have revolutionized generative modeling by facilitating high-quality image generation through an iterative refinement process that efficiently denoises images, maintaining excellence across diverse datasets like ImageNet. Building upon this, Normalizing Flows, introduced by Rezende and Mohamed in 2015, have further refined the field by enabling modeling of complex distributions with simpler, invertible transformations that enhance sampling efficiency and accelerate training. Extending these innovations, the Diffusion Transformer (DiT) leverages Transformer architecture to advance language processing and adapt to a broad spectrum of computer vision tasks by replacing the traditional convolutional U-Net with a more scalable and efficient transformer-based structure, proving particularly effective in transforming text into high-quality images and enhancing real-time generative applications.






\subsection{Text-to-Image Diffusion Models} %SD, SDXL, SD3, PixelArt 
Text-to-image diffusion models have rapidly evolved, featuring significant contributions from models such as Stable Diffusion (SD), SDXL, SD3, and Pixart-Alpha. These models have introduced unique techniques and innovations that substantially enhance their capability to generate detailed and contextually accurate images from textual descriptions. Stable Diffusion employs a Latent Diffusion Model (LDM) operating within a compressed latent space. This approach allows the model to efficiently generate high-quality images while minimizing computational demands. The efficiency of a compressed latent space facilitates faster processing times with minimal loss in image quality \cite{}. SDXL extends Stable Diffusion by incorporating an expanded U-Net architecture along with sophisticated text encoders such as CLIP. This enhancement improves the alignment between the generated images and the descriptive text, thus enhancing the model's ability to produce accurate visual representations of textual descriptions. The integration of CLIP enhances the model's understanding of textual nuances, leading to improved fidelity in visual outputs \cite{}. SD3 introduces further optimizations in the diffusion process through advanced training techniques and architectural improvements. These modifications aim to refine the model's output, enhance image fidelity, and expand the diversity of visual results. Such advancements contribute to more nuanced and detailed image generation capabilities, setting new benchmarks for image quality within the field \cite{}. Pixart-Alpha significantly advances the integration of multimodal inputs. This model modifies the standard diffusion process to optimize detail handling and better integrate text and image data. Pixart-Alpha's methodological adjustments allow it to excel in complex image synthesis tasks, particularly where fine details and high fidelity are crucial. These adjustments focus on enhancing the model's ability to interpret and visualize intricate details more effectively \cite{}.


\subsection{Few-Step Image Generation} %EMD, PD, LCM
Subsequent advancements in few-step image generation have introduced methods that significantly reduce computational demands. Enhanced Multiscale Diffusion (EMD) strategies, for example, initiate image generation from coarse resolutions and refine detail through fewer diffusion steps than traditional models, efficiently managing the scaling of image features. Progressive Distillation (PD) focuses on training smaller models that emulate the behavior of larger, pre-trained generative models, thereby reducing the number of diffusion steps required and accelerating the generation process. Latent Consistency Models (LCM), developed by Yang Song and colleagues, revolutionize this space by mapping noise directly to data through a learned consistency function, supporting one-step generation from noise and eliminating traditional iterative processes. These models can be trained either through distillation from existing diffusion models or independently, marking them as versatile tools in generative modeling.


\subsection{Post Training} 

%  DDPMs consists of two stages - a forward process and a reverse process. In the forward process, a clean image, denoted as \( x_0 \), is initially sampled. Subsequently, incremental Gaussian noises with a predefined variance schedule \(\{ \beta_1, \ldots, \beta_T \}\) are added sequentially over \( T \) timesteps. The overall forward process encompasses this series of operations, with each step explicitly defined by the addition of noise according to the schedule. Each step in this process is given by,
% \begin{align}
%     q(x_t \mid x_{t-1}) = \mathcal{N}\left(x_t; \sqrt{(1 - \beta_t}x_{t-1}, \beta_t \mathbf{I}\right) \label{eq:ddpm} \\
%     \Rightarrow x_t= \sqrt{1-\beta_t} x_{t-1} + \sqrt{\beta_t} \epsilon_t,    
%     \epsilon_t \sim \mathcal{N}(0, \mathbf{I}) \label{eq:ddpm_1}
% \end{align}

% In this formula, by writing \( \alpha_t=1 - \beta_t \), and \( \bar \alpha_t= \prod_{i=0}^T \alpha_i \), we have
% \begin{align}
%     q(x_t \mid x_0) = \mathcal{N}\left(x_0; \sqrt{\bar \alpha_t} x_0, (1-\bar \alpha_t) \mathbf{I}\right) \label{eq:ddpm} \\
%     \Rightarrow x_t= \sqrt{\bar \alpha_t} x_0 + \sqrt{1-\bar \alpha_t} \epsilon_t, 
%     \epsilon_t \sim \mathcal{N}(0, \mathbf{I}) \label{eq:ddpm_1}
% \end{align}

% Conversely, the reverse process reconstructs the original data from the noise, aimed at reversing the noise additions made during the forward process. It's modeled by a neural network with parameters \( \theta \) to predicted \(\mu_\theta(x_t, t)\),
% \begin{align}
%     p_\theta(x_{t-1} \mid x_t) &:= \mathcal{N}(x_{t-1}; \mu_\theta(x_t, t), \hat{\beta_t} \mathbf{I})
% \end{align}

% For training the model, setting 
% \begin{align}
%     \mu_{\theta}(x_t, t) = \frac{1}{\sqrt{\alpha_t}} \left( x_t - \frac{\beta_t}{\sqrt{1 - \overline{\alpha_t}}} \epsilon_{\theta}(x_t, t) \right)
% \end{align}

% We could minimize the variational lower bound of the the negative log likelihood of the distribution of clean images \( x_0 \). This objective can be simplified as follows:
% \begin{align}
% \mathcal{L}(\theta) = \mathbb{E}_{x_0, \epsilon, t} \left[ \| \epsilon - \epsilon_{\theta}(x_t, t) \|^2 \right],
% \end{align}

% where \( \epsilon \) represents the noise added during the forward process, and \( \epsilon_{\theta}(x_t, t) \) is the noise predicted by the model.
 
